Machine Generation and Detection of Arabic Manipulated and Fake News

Fake news and deceptive machine-generated text are serious problems threatening modern societies, including in the Arab world. This motivates work on detecting false and manipulated stories online. However, a bottleneck for this research is lack of sufficient data to train detection models. We present a novel method for automatically generating Arabic manipulated (and potentially fake) news stories. Our method is simple and only depends on availability of true stories, which are abundant online, and a part of speech tagger (POS). To facilitate future work, we dispense with both of these requirements altogether by providing AraNews, a novel and large POS-tagged news dataset that can be used off-the-shelf. Using stories generated based on AraNews, we carry out a human annotation study that casts light on the effects of machine manipulation on text veracity. The study also measures human ability to detect Arabic machine manipulated text generated by our method. Finally, we develop the first models for detecting manipulated Arabic news and achieve state-of-the-art results on Arabic fake news detection (macro F1=70.06). Our models and data are publicly available.

==> Tables/Avg_Excluded_Words.tex <==
\begin{table}[h]
 \centering
 \footnotesize
\begin{tabular}[h]{ccc}
\hline 
 {\textbf{Words}}& &{\textbf{POS Tags}} \\
\hline 
\<محرز >&$\rightarrow$&
NOUN\_PROPER\\
 \<ينتقل > &$\rightarrow$
 &  VERB\\ %IV3MS
 \<الى > &$\rightarrow$& PREP \\
 \<برشلونة > &$\rightarrow$ &NOUN\_PROPER\\
 \<مقابل > &$\rightarrow$& NOUN  \\
120  &$\rightarrow$& NUM \\
\<مليون > &$\rightarrow$& NOUN   \\
 \<دولار> &$\rightarrow$&
 NOUN \\
\hline
\end{tabular} 
\caption{Avrage number of $k$-closest words excluded in each POS class} \label{tab:pos}
\end{table} 

==> Tables/News_Stat.tex <==
%MAM: I moved this to the Appendix


==> Tables/exp_tabels.tex <==
\begin{tabular}{cc}
    \begin{minipage}{.5\linewidth}

\begin{adjustbox}{width=9cm}

\renewcommand{\arraystretch}{1}
{
\raggedright
\scriptsize
\begin{tabular}{c||r}

\toprule
 \textbf{Subs. with $5$-closest of 	\colorbox{blue!10}{\<برشلونة>} }&  \textbf{Subs. with  $5$-closest of  \colorbox{blue!10}{\<برشلونة>},	\colorbox{orange!30}{\< محرز >}	 ~~and 	\colorbox{red!30}{120}}  \\ \toprule




\<دولار> 	\<مليون> 	120	\<مقابل> 	\colorbox{blue!10}{\<مدريد>}	\<الى> 	\<ينتقل> 	\<محرز> 	& 



\<دولار> 	\<مليون> 	\colorbox{red!20}{350}	\<مقابل> 	\colorbox{blue!10}{\<ليدز>}	\<الى> 	\<ينتقل> 	\colorbox{orange!30}{\<صلاح>}	\\


\<دولار> 	\<مليون> 	120	\<مقابل> 	\colorbox{blue!10}{\<باريس>}	\<الى> 	\<ينتقل> 	\<محرز> 	& 

\<دولار> 	\<مليون> 	\colorbox{red!20}{450}	\<مقابل> 	\colorbox{blue!10}{\<مدريد>}	\<الى> 	\<ينتقل> 	\colorbox{orange!30}{\<ميسي>}	\\



\<دولار> 	\<مليون> 	120	\<مقابل> 	\colorbox{blue!10}{\<فالنسيا>}	\<الى> 	\<ينتقل> 	\<محرز> 	& 

\<دولار> 	\<مليون> 	\colorbox{red!20}{155}	\<مقابل> 	\colorbox{blue!10}{\<باريس>}	\<الى> 	\<ينتقل> 	\colorbox{orange!30}{\<رونالدو>}	\\



\<دولار> 	\<مليون> 	120	\<مقابل> 	\colorbox{blue!10}{\<ميلان>}	\<الى> 	\<ينتقل> 	\<محرز> 	& 

\<دولار> 	\<مليون> 	\colorbox{red!20}{280}	\<مقابل> 	\colorbox{blue!10}{\<فالنسيا>}	\<الى> 	\<ينتقل> 	\colorbox{orange!30}{\<ماني>}	\\




\<دولار> 	\<مليون> 	120	\<مقابل> 	\colorbox{blue!10}{\<مانشستر>}	\<الى> 	\<ينتقل> 	\<محرز> &   

\<دولار> 	\<مليون> 	\colorbox{red!20}{70}	\<مقابل> 	\colorbox{blue!10}{\<مرسيليا>}	\<الى> 	\<ينتقل> 	\colorbox{orange!30}{\<غويرو>}	\\


\toprule

\end{tabular}
} \end{adjustbox}
    \end{minipage} &

    \begin{minipage}{.3\linewidth}

\small    
\begin{tabular}[h]{ccc}
\hline 
 {\textbf{Words}}& &{\textbf{POS Tags}} \\
\hline 
\<محرز >&$\rightarrow$&
NOUN\_PROP\\
 \<ينتقل > &$\rightarrow$
 &  VERB\\ %IV3MS
\<الى > &$\rightarrow$& PREP \\
 \<برشلونة > &$\rightarrow$ &NOUN\_PROP\\
 \<مقابل > &$\rightarrow$& NOUN  \\
120  &$\rightarrow$& NUM \\
\<مليون > &$\rightarrow$& NOUN   \\
 \<دولار> &$\rightarrow$&
 NOUN \\
\hline
\end{tabular} 
    \end{minipage} 
\end{tabular}

==> Tables/pos_stat.tex <==
 \begin{table}[h]


\begin{center}


 \begin{tabular}{llll}
 \toprule
Label\_POS & Count  & Avg  & Median \\
\toprule
ADJ        & 99,538 & 3.79   & 3.00   \\
ADJ\_COMP  & 4,513  & 2.81   & 2.00   \\
ADJ\_NUM   & 5,752  & 3.06   & 3.00   \\
NOUN\_NUM  & 60,615 & 0.55   &  0.00   \\
NOUN\_PROP & 75,771 & 2.93   & 2.00  \\
\toprule
\end{tabular}
\caption{Descriptive statistics of k-closest words excluded in each POS clas. We note that the \textbf{NEG\_PART} is absent in the table, because we simply remove it from the sentence, so the  word embeddings model is not used in this case.\\}  \label{tab:pos_exc}
\end{center}
    \end{table}
 
 
 \begin{table}[]

\end{table}

==> Tables/save_tab.tex <==
 &   & & Rue20 &  $36,556$  &  \\
&   & &Khabarmaroc &    $2,196$ &\\
&& &   Yabiladi &  $28,760$ &\\
Morocco & 7 &&  Albidaoui& $14,019$ &  $178,911$   \\
&&&  Assdae & $18,600$  &  \\
&& & Assabah & $68,564$ &   \\
&&&    Alakhbarpressma&  $1,021$ & \\  \hline

 


&&  & Echoroukonline &  $187,936$  &  \\
&&&  Elkhabar & $121,441$  &  \\
Algeria & 6 & &  Ech chaab& $147,960$&      $520,162$    \\
&&   &el-massa &    $59,917$ &\\
&&&  Eljadidelyawmi & $2,556$ &  \\
&&&  Alomah &$352$&  \\ \hline


		
&&  & Aljarida &  $44,354$  & \\
&&  & Assarih &  $99,468$  &  \\
Tunisia&5&   &	Lemaghreb	 &   $76,550$  & \\
 && &	Hakaekonline &	$128,553$&    $451,278 $  \\
 &  &&  	Alchourouk	& $102,353$&     \\\hline


							
	

&&  & Elyom	 &  $22,993$  &  \\
&&   &Alahalygate &	$25,235$ &\\
Egypt &5& & 	Akhbarway&	$80,561$&   $3,021,352$    \\
 &  &&  	Soutalomma	& $133,128$&     \\
&&&  youm7 &	$2,759,435$  &  \\ \hline



 && & 	an7a	 &   $70,985$    \\
 &  &&  	Alriyadh	& $212,666$&     \\ 
 
Saudi&5&&  Uqngovsa &	 $20,994$ & $304,899$ \\
&&  & Alhadath	 &  $220$  & \\
&&   &Aljazeera &	$34$ & \\ \hline


 && & 	Sadaalshaamnet	 &   $12,994$    \\
Syria & 3 &  &	Alwatansy	& $10,468$& $47,058$    \\ 
 
&&  & Ayyamsyrianet &	 $23,578$ &  \\ \hline



 && & 	Alsudaninews	 &   $11,153$    \\
Syria & 3 &  &	Alwatansy	& $104,68$& $47,058$    \\ 
&&  & Ayyamsyrianet &	 $23,578$ &  \\ \hline


 &&   & 	Sadaalshaamnet	 &   $12,994$    \\
Sudan & 3 &  &	Alsudanalyoum	& $10,1924$ & $113,121$   \\ 
&&  & Alwandaily &	 $44$ &  \\ \hline


& & &Alsharaeanews&$1,261$  \\
Yemen& 3& &Alsomoud&$94,86$ & $83,802$\\
& & &Althawrah&$73,055$ \\ \hline

&  & & Beiruttimes&$9,629$  & $99,080$\\
USA&2  & &Sadaalwatan&$11,091$ \\   
& & &Watanserb&$78,360$ \\  \hline 



UK& 2 & &Watanserb&$78360$ & $295566$ \\
& & &Middleeastonline&$295190$ \\ \hline

UAE & 2 & &BBC& $5471$ & $63897$\\ 
& & &Elbyan&$58426$ \\ \hline

Iraq & 1 & & Alayam &  $120,311$ & $120,311$ \\ \hline

Kuwait& 1&   &Azzaman&  $31354$  & $31354$\\ \hline

Jordan& 1 &  &Alwasat&  $689,444$  & $689,444$ \\ \hline

Lebanon& 1  &   &Addustour&$42,388$  & $42,388$\\ \hline


Palestine& 1 & &arab48&$35,286$ & $35,286$\\\hline 

Bahrain& 1  &   &Addustour&$7,612$  & $7,612$\\ \hline


